Framing Visual Musicology through Methodology Transfer

In this position paper, we frame the field of Visual Musicology by providing an overview of well-established musicological sub-domains and their corresponding analytic and visualization tasks. To foster collaborative, interdisciplinary research, we discuss relevant data and domain characteristics. We give a description of the problem space, as well as the design space of musicology and discuss how existing problem-design mappings or solutions from other fields can be transferred to musicology. We argue that, through methodology transfer, established methods can be exploited to solve current musicological problems and show exemplary mappings from analytics fields related to text, geospatial, time-series, and other high-dimensional data to musicology. Finally, we point out open challenges, discuss research gaps, and highlight future research opportunities.

==> files/notes.tex <==

% Was ist unser Position Statement?!
% Wie machen wir die Leute auf uns aufmerksam nd motivieren sie etwas zu tun.
% Visual Musicology is a new field of research -> win-win-situation 
% Commonalities, Sequence Data, Existing data types and solutions/visualizations
% Visual Musicology present a new term

% Related 

